Empower Large Language Model to Perform Better on Industrial Domain-Specific Question Answering

Large Language Model (LLM) has gained popularity and achieved remarkable results in open-domain tasks, but its performance in real industrial domain-specific scenarios is average due to its lack of specific domain knowledge. This issue has attracted widespread attention, but there are few relevant benchmarks available. In this paper, we provide a benchmark Question Answering (QA) dataset named MSQA, centered around Microsoft products and IT technical problems encountered by customers. This dataset contains industry cloud-specific QA knowledge, an area not extensively covered in general LLMs, making it well-suited for evaluating methods aiming to enhance LLMs' domain-specific capabilities. In addition, we propose a new model interaction paradigm that can empower LLM to achieve better performance on domain-specific tasks where it is not proficient. Extensive experiments demonstrate that the approach following our method outperforms the commonly used LLM with retrieval methods. We make our source code and sample data available at: https://aka.ms/Microsoft_QA.

==> main/CaseStudy.tex <==
\section{Case Study}


Table ~\ref{tab:case} presents a comparison of GPT-4 responses before and after three knowledge-enhancement methods. 
For typographical considerations, we present only a portion of the key information here and use ellipses to replace the remaining content.
It can be observed that  GPT-4, without any knowledge augmentation, struggles to comprehend the meaning of "price" within the question, subsequently failing to provide an answer. The retrieval-based augmentation method (BM25) did not provide any additional useful information, which resulted in {GPT-4 + BM25} still being unable to answer the user. However, the two responses of GPT-4 enhanced by expert opinions, i.e., {GPT-4 + Expert} and {GPT-4 + Expert \& BM25}, both correctly answered the question. This demonstrates the effectiveness of the model fusion framework proposed in this work. Comparing the responses of GPT-4 enhanced by expert opinions and the expert opinions itself, "\textit{The price is included in the composed model fee}" from GPT-4 is semantically closer to "\textit{No extra fee}" than "\textit{The price is the price of the composed model}" from the expert.
